A Survey on Vertical Federated Learning: From a Layered Perspective

Vertical federated learning (VFL) is a promising category of federated learning for the scenario where data is vertically partitioned and distributed among parties. VFL enriches the description of samples using features from different parties to improve model capacity. Compared with horizontal federated learning, in most cases, VFL is applied in the commercial cooperation scenario of companies. Therefore, VFL contains tremendous business values. In the past few years, VFL has attracted more and more attention in both academia and industry. In this paper, we systematically investigate the current work of VFL from a layered perspective. From the hardware layer to the vertical federated system layer, researchers contribute to various aspects of VFL. Moreover, the application of VFL has covered a wide range of areas, e.g., finance, healthcare, etc. At each layer, we categorize the existing work and explore the challenges for the convenience of further research and development of VFL. Especially, we design a novel MOSP tree taxonomy to analyze the core component of VFL, i.e., secure vertical federated machine learning algorithm. Our taxonomy considers four dimensions, i.e., machine learning model (M), protection object (O), security model (S), and privacy-preserving protocol (P), and provides a comprehensive investigation.

==> sections/algorithm_design.tex <==
\section{Machine Learning Algorithm Design of VFL}
\label{sec:algorithm_design}
 
\begin{table*}[ht]
\centering
\begin{tabular}{ccc}
\toprule
 & Machine learning model & Existing work \\
\midrule
\multirow{5}{*}{Vertical supervised learning model} & Vertical linear model & \cite{gascon2017privacy}, \cite{yang2019parallel}, \cite{wei2021privacy}, \cite{yang2019quasi}, \cite{zhang2021secure}, \cite{zhang2021asysqn}\\
& Vertical kernel model & \cite{gu2020federated},\cite{dang2020large}, \cite{yu2006privacy},
	\cite{atarashi2021vertical}\\
& Vertical tree model & \cite{vaidya2008privacy}, \cite{cheng2021secureboost}, \cite{fu2021vf2boost}, \cite{wu2020privacy}, \cite{khodaparast2018privacy}, \cite{feng2019securegbm}, \cite{le2021fedxgboost}, \cite{fang2021large}, \cite{zhu2021pivodl}\\
& Vertical neural network & \cite{vepakomma2018split}, \cite{zhu2021from}, \cite{liu2020federated}, \cite{liang2021self},
	\cite{cha2021implementing},
	\cite{fu2022label}\\
%Support Vector Machine & \cite{yu2006privacy}, \cite{ge2021failure}\\
& Vertical graph neural network & \cite{ni2021vertical}, \cite{zhang2021federated}, \cite{cheung2021fedsgc}, \cite{zhou2020vertically},
	\cite{chen2022graph}\\
\midrule
Vertical semi-supervised learning model &~\makecell[c]{multi-view learning, Split-NN, GAN,\\knowledge distillation, self-taught learning}&~\cite{kang2022fedcvt},~\cite{wu2021exploiting},~\cite{peng2021differentially},~\cite{zhang2022data},~\cite{ren2021improving},~\cite{chu2021privacy}\\
\midrule
Vertical unsupervised learning model &~\makecell[c]{K-means clustering, hierarchical clustering,\\principal component analysis, self-organizing maps} &~\cite{vaidya2003privacy},~\cite{sheikhalishahi2017privacy},~\cite{cheung2022vertical},~\cite{kholod2021parallelization}\\
\bottomrule
\end{tabular}
\caption{Summary of vertical machine learning models studied in vertical federated learning.}
\label{tab:mlmodel-vfl}
\end{table*}

%\begin{landscape}
%\begin{figure}
%\centering
%\begin{forest}
%forked edges,
%for tree={draw,align=center,edge={-latex}},
%where level=3{
%  folder,
%  grow'=0,
%  yshift=75pt,
%}{}
%[\textbf{Vertical federated learning}
%  [\textbf{Semi-honest}\\~\textbf{\& colluding}
%    [\textbf{Data~\& model privacy}
%      [\textbf{MPC-based}\\~\textbf{protection}
%        [\textit{Tree models}\\~\cite{vaidya2008privacy}]
%      ]
%      [\textbf{Other}\\~\textbf{protection}
%        [\textit{Linear models}\\~\cite{zhang2021asysqn}]
%      ]
%    ]
%  ]
%  [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%    [\textbf{Data~\& model privacy}
%      [\textbf{HE-based}\\~\textbf{protection}
%        [\textit{Linear models}\\~\cite{yang2019federated}~\cite{yang2021model}~\cite{wei2021privacy}\\~\cite{yang2019parallel}~\cite{yang2019quasi}]
%        [\textit{Mixture models}\\~\cite{ou2020homomorphic}]
%        [\textit{Tree models}\\~\cite{cheng2021secureboost}~\cite{feng2019securegbm}~\cite{fu2021vf2boost}\\~\cite{wu2020privacy}~\cite{zhu2021pivodl}]
%        [\textit{Neural networks}\\~\cite{zhang2020additively}]
%        [\textit{Graph models}\\~\cite{ni2021vertical}]
%      ]
%      [\textbf{MPC-based}\\~\textbf{protection}
%        [\textit{Linear models}\\~\cite{gascon2017privacy}~\cite{zhang2021secure}~\cite{chen2021homomorphic}\\~\cite{mohassel2017secureml}~\cite{mohassel2018aby3}]
%        [\textit{Kernel models}\\~\cite{gu2020federated}~\cite{dang2020large}~\cite{yu2006privacy}]
%        [\textit{Tree models}\\~\cite{khodaparast2018privacy}~\cite{le2021fedxgboost}~\cite{fang2021large}]
%        [\textit{Neural networks}\\~\cite{mohassel2017secureml}~\cite{huang2022cheetah}~\cite{mohassel2018aby3}]
%      ]
%      [\textbf{DP-based}\\~\textbf{protection}
%        [\textit{Linear models}\\~\cite{xu2019achieving}~\cite{wang2020hybrid}]
%        [\textit{Tree models}\\~\cite{le2021fedxgboost}~\cite{zhu2021pivodl}]
%        [\textit{Neural networks}\\~\cite{yang2022differentially}~\cite{liang2021self}]
%        [\textit{Graph models}\\~\cite{peng2021differentially}]
%      ]
%      [\textbf{Other}\\~\textbf{protection}
%        [\textit{Linear models}\\~\cite{li2016vertical}~\cite{kim2021vertical}~\cite{hu2019fdml}]
%        [\textit{Kernel models}\\~\cite{yunhong2009privacy}~\cite{atarashi2021vertical}]
%        [\textit{Neural networks}\\~\cite{hu2019fdml}~\cite{cha2021implementing}~\cite{vepakomma2018split}\\~\cite{liu2020federated}~\cite{cha2021implementing}]
%      ]
%    ]
%%    [\textbf{Model privacy}\\~\cite{gu2020federated}~\cite{dang2020large}]
%    [\textbf{Model utility}]
%    [\textbf{Model security}]    
%  ]
%  [\textbf{Malicious}\\~\textbf{\& colluding}]
%  [\textbf{Malicious}\\~\textbf{\& non-colluding}
%    [\textbf{Data \& model privacy}
%      [\textbf{MPC-based}\\~\textbf{protection}
%        [\textit{Linear models}\\~\cite{mohassel2018aby3}~\cite{dalskov2021fantastic}]
%        [\textit{Neural networks}\\~\cite{mohassel2018aby3}~\cite{dalskov2021fantastic}]
%      ]
%    ]
%  ]
%]
%\end{forest}
%\end{figure}
%\end{landscape}

%\begin{figure*}
%\centering
%\small
%\begin{forest}
%forked edges,
%for tree={draw,align=center,edge={-latex},grow'=0},
%[\textbf{Secure vertical}\\~\textbf{federated learning}\\~\textbf{algorithm}
%  [\textbf{Linear model}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textbf{HE-based protocol}:~\cite{yang2019federated}~\cite{yang2021model}~\cite{wei2021privacy}\\~\cite{yang2019parallel}~\cite{yang2019quasi}]
%        [\textbf{MPC-based protocol}:~\cite{gascon2017privacy}~\cite{chen2021homomorphic}\\~\cite{demmler2015aby}~\cite{mohassel2017secureml}~\cite{mohassel2018aby3}]
%        [\textbf{DP-based protocol}:~\cite{xu2019achieving}~\cite{wang2020hybrid}~\cite{luo2021feature}~\cite{jiang2022comprehensive}]
%        [\textbf{Other protocols}:~\cite{li2016vertical}~\cite{kim2021vertical}~\cite{hu2019fdml}~\cite{zhang2021asysqn}\\~\cite{zhang2021secure}~\cite{zhang2021desirable}]
%      ]
%      [\textbf{Semi-honest}\\~\textbf{\& colluding}
%      	[\textbf{HE-based protocol}:~\cite{weng2020privacy}]
%        [\textbf{Other protocols}:~\cite{zhang2021asysqn}~\cite{zhang2021secure}~\cite{zhang2021desirable}]
%      ]
%      [\textbf{Malicious}\\~\textbf{\& non-colluding}
%        [\textbf{MPC-based protocol}:~\cite{mohassel2018aby3}~\cite{dalskov2021fantastic}]
%        [\textbf{Other protocols}:~\cite{zhang2021desirable}]
%      ]
%    ]
%    [\textbf{Model security}
%      [\textbf{Malicious}\\~\textbf{\& non-colluding}
%        [\textbf{Other protocols}:~\cite{zhang2021desirable}~\cite{liu2020backdoor}]
%      ]
%    ]f
%  ]
%  [\textbf{Tree model}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textbf{HE-based protocol}:~\cite{cheng2021secureboost}~\cite{feng2019securegbm}~\cite{fu2021vf2boost}\\~\cite{wu2020privacy}~\cite{zhu2021pivodl}]
%        [\textbf{MPC-based protocol}:~\cite{khodaparast2018privacy}~\cite{le2021fedxgboost}~\cite{fang2021large}\\~\cite{sheikhalishahi2017privacy}]
%        [\textbf{DP-based protocol}:~\cite{le2021fedxgboost}~\cite{zhu2021pivodl}~\cite{luo2021feature}~\cite{jiang2022comprehensive}]
%      ]
%      [\textbf{Semi-honest}\\~\textbf{\& colluding}
%        [\textbf{MPC-based protocol}:~\cite{vaidya2008privacy}]
%      ]
%      [\textbf{Malicious}\\~\textbf{\& non-colluding}
%      	[\textbf{HE-based protocol}:~\cite{weng2020privacy}]
%      ]
%    ]
%  ]
%  [\textbf{Neural network}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textbf{HE-based protocol}:~\cite{zhang2020additively}]
%        [\textbf{MPC-based protocol}:~\cite{mohassel2017secureml}~\cite{huang2022cheetah}~\cite{mohassel2018aby3}]
%        [\textbf{DP-based protocol}:~\cite{yang2022differentially}~\cite{liang2021self}~\cite{luo2021feature}~\cite{jiang2022comprehensive}]
%        [\textbf{Other protocols}:~\cite{hu2019fdml}~\cite{cha2021implementing}~\cite{vepakomma2018split}\\~\cite{liu2020federated}~\cite{cha2021implementing}~\cite{kang2022fedcvt}~\cite{wu2021exploiting}~\cite{zhang2022data}~\cite{ren2021improving}\\~\cite{chu2021privacy}~\cite{kholod2021parallelization}~\cite{zhang2021desirable}]
%      ]
%      [\textbf{Semi-honest}\\~\textbf{\& colluding}
%        [\textbf{Other protocols}:~\cite{zhang2021desirable}]
%      ]
%      [\textbf{Malicious}\\~\textbf{\& non-colluding}
%        [\textbf{MPC-based protocol}:~\cite{mohassel2018aby3}~\cite{dalskov2021fantastic}]
%        [\textbf{Other protocols}:~\cite{zhang2021desirable}]
%      ]
%    ]
%    [\textbf{Model security}
%      [\textbf{Malicious}\\~\textbf{\& non-colluding}
%        [\textbf{Other protocols}:~\cite{zhang2021desirable}~\cite{liu2020backdoor}]
%      ]
%    ]
%  ]
%%  [\textbf{Graph model}
%%    [\textbf{Data \& model}\\~\textbf{privacy}
%%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%%        [\textbf{HE-based protocol}\\~\cite{ni2021vertical}~\cite{cheung2021fedsgc}]
%%        [\textbf{DP-based protocol}\\~\cite{zhou2020vertically}~\cite{peng2021differentially}]
%%      ]
%%    ]
%%  ]
%  [\textbf{Other models}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textbf{HE-based protocol}:~\cite{ou2020homomorphic}~\cite{ni2021vertical}~\cite{cheung2021fedsgc}]
%        [\textbf{MPC-based protocol}:~\cite{dang2020large}\\~\cite{yu2006privacy}~\cite{vaidya2003privacy}~\cite{chen2020secure}]
%        [\textbf{DP-based protocol}:~\cite{zhou2020vertically}~\cite{peng2021differentially}]
%        [\textbf{Other protocols}:~\cite{yunhong2009privacy}~\cite{atarashi2021vertical}~\cite{cheung2022vertical}\\~\cite{gu2020federated}]
%      ]
%    ]
%  ]
%]
%\end{forest}
%\caption{The categorization of existing secure vertical federated learning algorithms.}
%\label{fig:cate_VFL}
%\end{figure*}


%\begin{figure*}
%\centering
%\begin{forest}
%forked edges,
%for tree={draw,align=center,edge={-latex},grow'=0},
%[\textbf{Vertical federated}\\~\textbf{unsupervised learning}
%  [\textbf{Vertical}\\~\textbf{K-means}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textit{MPC-based protection}\\~\cite{vaidya2003privacy}]
%      ]
%    ]
%  ]
%  [\textbf{Vertical}\\~\textbf{PCA}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textit{Other protection}\\~\cite{cheung2022vertical}]
%      ]
%    ]
%  ]
%  [\textbf{Vertical}\\~\textbf{matrix factorization}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textit{MPC-based protection}\\~\cite{chen2020secure}]
%      ]
%    ]
%  ]
%  [\textbf{Vertical}\\~\textbf{mixture model}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textit{HE-based protection}\\~\cite{ou2020homomorphic}]
%      ]
%    ]
%  ]
%  [\textbf{Vertical}\\~\textbf{tree model}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textit{MPC-based protection}\\~\cite{sheikhalishahi2017privacy}]
%      ]
%    ]
%  ]
%  [\textbf{Vertical}\\~\textbf{neural network}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textit{Other protection}\\~\cite{kholod2021parallelization}]
%      ]
%    ]
%  ]
%  [\textbf{Vertical}\\~\textbf{graph model}
%    [\textbf{Data \& model}\\~\textbf{privacy}
%      [\textbf{Semi-honest}\\~\textbf{\& non-colluding}
%        [\textit{DP-based protection}\\~\cite{peng2021differentially}]
%      ]
%    ]
%  ]
%]
%\end{forest}
%\end{figure*}

%In this section, we summarize existing efforts in designing machine learning algorithms in VFL. Specifically, we divide the algorithms into machine learning models and optimization methods.

%\subsection{Vertical Machine Learning Model}
%Machine learning model $f$ maps the input features $\mathbf{X}$ into desired outputs, such as predicted labels $\hat{\mathbf{y}}$ for supervised learning. We consider three classes of machine learning models,~\ie, supervised, semi-supervised, and unsupervised learning models.
%, shown in Tab.~\ref{tab:mlmodel-vfl}.

%\subsubsection{Vertical Supervised Learning Model}
%Supervised learning models are arguably the most studied models in VFL. Given input features $\mathbf{X}$ (\eg, an image) and labels $\mathbf{y}$ (\eg, +1/-1 for binary classification), supervised learning models aim to learn a model $f(\mathbf{X} | \bm{\theta})$ to map input features to labels correctly. Many classes of supervised learning models have been studied in the context of VFL.

%\paragraph{Vertical Kernel Model}




%\subsubsection{Vertical Semi-Supervised Learning Model}


%\paragraph{Self-Supervision-Based Model~\highlight{do not know if the name is proper}}

% while self-supervision-based methods aim to learn feature representations using non-overlapping data to complement supervised training.

%Unlike similarity-based models that aim to borrow features from other parties, self-supervision-based models focus on utilizing non-overlapping samples of each party independently. One way of utilizing them is to use all samples at each party to learn features using self-supervised learning, such that the overall model is complemented with latent structures of non-overlapping samples. 

\subsubsection{Vertical Unsupervised Learning Model}

%2006 PAKDD: Privacy-preserving svm classification on vertically partitioned data~\cite{yu2006privacy}
%   	\begin{itemize}
%   		\item Vertical federated SVM for classification problems using secret sharing
%   		\item includes both linear and non-linear kernels
%   	\end{itemize}


%2017 Proc. Priv. Enhancing Technol.: Privacy-Preserving Distributed Linear Regression on High-Dimensional Data~\cite{gascon2017privacy}
%        \begin{itemize}
%            \item hybrid multi-party computation protocol that combines Yao’s garbled circuits with tailored protocols for computing inner products.
%        \end{itemize}
        
%TIST: Federated Machine Learning: Concept and Applications~\cite{yang2019federated}
%        \begin{itemize}
%            \item first to introduce the notion of VFL.
%        \end{itemize}

%2019 FL-IJCAI: Parallel Distributed Logistic Regression for Vertical Federated Learning without Third-Party Coordinator~\cite{yang2019parallel}
%        \begin{itemize}
%            \item parallel distributed logistic regression for vertical federated learning.
%            \item the role of third-party coordinator is removed.
%            \item built on the parameter server architecture and aims to speed up the model training via utilizing a cluster of servers in case of large volume of training data.
%        \end{itemize}
        
%2019 ICLR AI for social good workshop: Split learning for health: Distributed deep learning without sharing raw patient data~\cite{vepakomma2018split}
%        \begin{itemize}
%            \item proposes the VFL configurations of SplitNN.
%        \end{itemize}

%2021 Peer-to-Peer Networking and Applications: Privacy-preserving two-parties logistic regression on vertically partitioned data using asynchronous gradient sharing~\cite{wei2021privacy}
%        \begin{itemize}
%            \item a protocol using that can complete the logistic regression modeling of vertically partitioned data by asynchronous gradient sharing.
%        \end{itemize}

%2020 VLDB: Privacy Preserving Vertical Federated Learning for Tree-based Models~\cite{wu2020privacy}
%        \begin{itemize}
%            \item propose Pivot, a novel solution for privacy preserving vertical decision tree training and prediction, ensuring that no intermediate information is disclosed other than those the clients have agreed to release.
%        \end{itemize}
        
%2018 DASC/PiCom/DataCom/CyberSciTech: Privacy Preserving Random Decision Tree Classification over Horizontally and Vertically Partitioned Data~\cite{khodaparast2018privacy}
%    \begin{itemize}
%        \item a framework for constructing Random Decision Trees on horizontally and vertically partitioned dataset.
%    \end{itemize}

%2019 Big Data: SecureGBM: Secure Multi-Party Gradient Boosting~\cite{feng2019securegbm}
%        \begin{itemize}
%            \item “dual- party”secure learning scenario based on two parties — both party own an unique view (i.e., attributes or features) to the sample group of samples while only one party owns the labels.
%            \item feature and label data are not allowed to share with others
%        \end{itemize}
        
%2021 arXiv: FedXGBoost: Privacy-Preserving XGBoost for Federated Learning~\cite{le2021fedxgboost}

%2018 Journal of Network and Computer Applications: Distributed learning of deep neural network over multiple agents~\cite{gupta2018distributed}
%        \begin{itemize}
%            \item split learning
%            \item health care and finance
%            \item shortage of labeled data and computational resources
%        \end{itemize}
        
%2020 KDD: Federated Doubly Stochastic Kernel Learning for Vertically Partitioned Data~\cite{gu2020federated}
%        \begin{itemize}
%            \item use nonlinear learning with kernels instead of traditional data mining and machine learning algorithms in order to train effectively and efficiently.
%        \end{itemize}
        
%2020 FLPI: Federated recommendation systems~\cite{yang2020federated}
%        \begin{itemize}
%            \item introduce a new notion of federated recommender systems, which is an instantiation of federated learning on decentralized recommendation..
%        \end{itemize}
        
%2020 FLPI: Large-Scale Kernel Method for Vertical Federated Learning~\cite{dang2020large}
%        \begin{itemize}
%            \item first approximate the kernel function by the random feature technique.
%            \item then federatedly update the predict function by the special designed doubly stochastic gradient without leaking privacy in both data and model.
%        \end{itemize}
        
%2021 IEEE Intelligent Systems: Secureboost: A lossless federated learning framework~\cite{cheng2021secureboost}
%        \begin{itemize}
%            \item constructs boosting trees across multiple parties with a carefully designed encryption strategy.
%            \item discuss information leakage during the protocol execution and propose ways to provably reduce it.
%        \end{itemize}
        
%2021 PAKDD: Vertical Federated Learning for Higher-Order Factorization Machines~\cite{atarashi2021vertical}
%        \begin{itemize}
%            \item VFL method for higher-order factorization machines
%        \end{itemize}
        
%2021 JMIR Medical Informatics: Implementing Vertical Federated Learning Using Autoencoders: Practical Application, Generalizability, and Utility Study~\cite{cha2021implementing}
%        \begin{itemize}
%            \item autoencoder-based ML model for vertically incomplete data.
%        \end{itemize}
        
%2021 SIGMOD: VF2Boost: Very Fast Vertical Federated Gradient Boosting for Cross-Enterprise Learning~\cite{fu2021vf2boost}
%        \begin{itemize}
%            \item a novel and efficient vertical federated GBDT system.
%            \item First, to handle the deficiency caused by frequent mutual-waiting in federated training, we propose a concurrent training protocol to reduce the idle periods.
%            \item Second, to speed up the cryptography operations, we analyze the characteristics of the algorithm and propose customized operations.
%        \end{itemize}
        
%2021 Journal of Intelligent Manufacturing: Failure prediction in production line based on federated learning: an empirical study~\cite{ge2021failure}
%        \begin{itemize}
%            \item application on failure prediction in the production line
%            \item Federated Support Vector Machine and federated random forest algorithms for the horizontal FL and vertical FL scenarios
%        \end{itemize}
        

%2021 Complex \& Intelligent Systems: From federated learning to federated neural architecture search: a survey~\cite{zhu2021from}
%        \begin{itemize}
%            \item neural architecture search about VFL
%            \item survey
%        \end{itemize}
        
%2020 AAAI: Federated learning for vision-and-language grounding problems~\cite{liu2020federated}
%        \begin{itemize}
%            \item a federated learning frame- work to obtain various types of image representations from different tasks, which are then fused together to form fine-grained image representations.
%            \item include vertical federated learning
%        \end{itemize}

%2021 arXiv: Self-supervised cross-silo federated neural architecture search~\cite{liang2021self}
%        \begin{itemize}
%            \item Self-supervised Vertical Federated Neural Architecture Search (SS-VFNAS) for automating FL where participants hold feature-partitioned data
%        \end{itemize}

%2021 arXiv: A Vertical Federated Learning Framework for Graph Convolutional Network~\cite{ni2021vertical}
%        \begin{itemize}
%            \item a federated GCN learning paradigm for privacy-preserving node classification task under data vertically partitioned setting
%        \end{itemize}
        
%2021 arXiv: Federated Graph Learning--A Position Paper~\cite{zhang2021federated}
%        \begin{itemize}
%            \item inter- graph FL, intra-graph FL and graph-structured FL
%            \item intra-graph is further divided into horizontal and vertical FGL
%        \end{itemize}

%\subsubsection{Semi-Supervised Learning Model}
%2020 FL-IJCAI: FedMVT: Semi-supervised Vertical Federated Learning with MultiView Training~\cite{kang2020fedmvt}
%        \begin{itemize}
%            \item limited overlapping samples.
%            \item estimates representations for missing features and predicts pseudo-labels for unlabeled samples.
%        \end{itemize}
        
% 2020 arXiv: Multi-participant multi-class vertical federated learning~\cite{feng2020multi}
%         \begin{itemize}
%            \item extending the idea of multi-view learning.
%            \item label sharing from its owner to other VFL participants in a privacy-preserving manner.
%        \end{itemize}

% \cite{cha2021implementing} proposes to use autoencoders to replace local DNNs for passive parties. Thus, each passive party can locally learn feature representations of their local data in addition to learning with labels from the active party. 

% 2021 arXiv: Privacy-Preserving Self-Taught Federated Learning for Heterogeneous Data~\cite{chu2021privacy}
%         \begin{itemize}
%             \item uses unsupervised feature extraction techniques for distributed supervised deep learning tasks
%             \item only latent variables are transmitted to other parties for model training, while privacy is preserved by storing the data and parameters of activations, weights, and biases locally.
%         \end{itemize}

% 2021 arXiv: Exploiting Record Similarity for Practical Vertical Federated Learning~\cite{wu2021exploiting}
%         \begin{itemize}
%             \item a novel similarity-based VFL framework.
%             \item study the “record linkage” process.
%             \item fuzzy matching.
%         \end{itemize}
        


% 2003 KDD: Privacy-preserving k-means clustering over vertically partitioned data~\cite{vaidya2003privacy}
%   	\begin{itemize}
%   		\item Privacy-preserving K-means for vertically partitioned data	
%   	\end{itemize}

% 2017 ISCC: Privacy preserving clustering over horizontal and vertical partitioned data~\cite{sheikhalishahi2017privacy}
%	\begin{itemize}
%		\item hierarchical clustering model for vertically partitioned data
%	\end{itemize}
	
% 2021 The Journal of Supercomputing: Parallelization of the self-organized maps algorithm for federated learning on distributed sources~\cite{kholod2021parallelization}
%        \begin{itemize}
%            \item parallelizing the Kohonen algorithm used for the federated learning process in a special kind of neural networks— Self-Organizing Maps
%            \item reduces the execution time of the algorithm, the network traffic, and the risk of an unauthorized access to the data during their transmission
%        \end{itemize}

%2020 Computer Science and Information Systems: A Homomorphic-encryption-based Vertical Federated Learning Scheme for Rick Management~\cite{ou2020homomorphic}
%        \begin{itemize}
%            \item vertical federated learning system for the for Bayesian machine learning with the homomorphic encryption.
%            \item lots of typos.
%        \end{itemize}
        
%2020 technical report: Federated-PCA on Vertical-Partitioned Data~\cite{cheung2020federated}
%        \begin{itemize}
%            \item reduce the dimensionality of sample data
%            \item efficiency of subsequent training work
%        \end{itemize}

        
%\subsubsection{Transfer Learning Model}

%2020 AAAI: Federated learning for vision-and-language grounding problems~\cite{liu2020federated}
%        \begin{itemize}
%            \item a federated learning frame- work to obtain various types of image representations from different tasks, which are then fused together to form fine-grained image representations.
%            \item include vertical federated learning
%        \end{itemize}

%Privacy-preserving Federated Adversarial Domain Adaptation over Feature Groups for Interpretability~\cite{kang2021privacy}

\subsection{Vertical Optimization Method}
\label{subsec:optimization}
%
%\begin{table}
%\centering
%\resizebox{\columnwidth}{!}{
%\begin{tabular}{ccc}
%\toprule
%	Categorization & Optimization Methods & VFL Papers \\
%	\midrule
%	\multirow{4}{*}{Gradient-based} & First-order Synchronous & \cite{yang2019federated}, \cite{gu2020federated}, \cite{nathan2017optimization}\\
%	& First-order Asynchronous & \cite{hu2019fdml}, \cite{gu2021privacy}, \cite{zhang2021secure}, \cite{liu2019communication}, \cite{wei2021privacy}\\
%	& Second-order & \cite{zhang2021asysqn}, \cite{yang2019quasi}, \cite{gascon2017privacy}\\
%	& Zero-order & \cite{zhang2021desirable}\\
%	\midrule
%	EM Algorithms & & \cite{ou2020homomorphic}\\
%	\bottomrule
%\end{tabular}}
%\caption{A Summary of Optimization Methods Studied in VFL}
%\label{tab:optim-vfl}
%\end{table}

%After a model $f(\mathbf{X}|\bm{\theta})$ is formulated, learning the model is to solve the minimization problem in Eq.~\ref{eqn:vfl-formulation}. Two class of optimization methods,~\ie, gradient-based methods and EM-based methods, are utilized in VFL. 
%We introduce both types of methods in VFL, as summarized in Table \ref{tab:optim-vfl}.
 
\subsubsection{Vertical Gradient-Based Method}
Gradient methods are commonly used to optimize discriminative machine learning models, such as neural networks, logistic regression,~\etc. Depending on the information involved to optimize $L(\bm{\theta})$, gradient-based methods can be further divided into first-order, second-order, and zero-order methods. 
%We introduce each of them in VFL as follows. Given an objective function $\min_\theta L(\bm{\theta})$ with parameters $\bm{\theta}$, gradient-based methods aim to minimize $L(\bm{\theta})$ using the gradients $\nabla_\theta L(\bm{\theta})$. In general cases when $L(\bm{\theta})$ is not convex or $\nabla_\theta L(\bm{\theta})=0$ does not have a closed form solution, iterative methods are often leveraged to solve the minimization. 

\paragraph{Vertical First-Order Method}

%First-order methods, including gradient descent, momentum methods, AdaGrad \cite{duchi2011adaptive}, Adam \cite{kingma2014adam} etc., are most widely used in optimizing machine learning models due to their empirical performance, time and memory efficiency. 


%2020 FL-ICML: VAFL: a Method of Vertical Asynchronous Federated Learning~\cite{chen2020vafl}
%        \begin{itemize}
%            \item each client to run stochastic gradient algorithms without coordination with other clients.
%            \item perturbed local embedding to ensure data privacy and improve communication efficiency.
%        \end{itemize}

%2019 FL-NeurIPS: A Quasi-Newton Method Based Vertical Federated Learning Framework for Logistic Regression~\cite{yang2019quasi}
%        \begin{itemize}
%            \item Existing frameworks adopt the first-order stochastic gradient descent algorithm.
%            \item propose a quasi-Newton method based vertical federated learning framework for logistic regression under the additively homomorphic encryption scheme.
%            \item reduce the number of communication rounds with a little additional communication cost per round.
%        \end{itemize}
        
%2019 FL-NeurIPS: A Communication Efficient Collaborative Learning Framework for Distributed Features~\cite{liu2019communication}
%        \begin{itemize}
%            \item each party conducts multiple local updates before each communication to effectively reduce the number of communication rounds among parties.
%        \end{itemize}

%2017 MLDM: Optimization for Large-Scale Machine Learning with Distributed Features and Observations~\cite{nathan2017optimization}
%		\begin{itemize}
%			\item doubly distributed optimization algorithms.
%		\end{itemize}
		
% 2017 Proc. Priv. Enhancing Technol.: Privacy-Preserving Distributed Linear Regression on High-Dimensional Data~\cite{gascon2017privacy}
%         \begin{itemize}
%             \item hybrid multi-party computation protocol that combines Yao’s garbled circuits with tailored protocols for computing inner products.
 %        \end{itemize}

%2019 KDD: FDML: A Collaborative Machine Learning Framework for Distributed Features~\cite{hu2019fdml}
%        \begin{itemize}
%            \item feature distributed machine learning scenario in Tencent.
%        \end{itemize}
        
%2020 KDD: Federated Doubly Stochastic Kernel Learning for Vertically Partitioned Data~\cite{gu2020federated}
%        \begin{itemize}
%            \item use nonlinear learning with kernels instead of traditional data mining and machine learning algorithms in order to train effectively and efficiently.
%        \end{itemize}
        
%2021 AAAI: Secure Bilevel Asynchronous Vertical Federated Learning with Backward Updating~\cite{zhang2021secure}
%        \begin{itemize}
%            \item most existing VFL algorithms are trapped in the synchronous computations, which leads to inefficiency in their real-world applications.
%            \item a novel VFL framework integrated with new backward updating mechanism and bilevel asynchronous parallel architecture.
%        \end{itemize}

%2021 IEEE Transactions on Neural Networks and Learning Systems: Privacy-Preserving Asynchronous Vertical Federated Learning Algorithms for Multiparty Collaborative Learning~\cite{gu2021privacy}
%        \begin{itemize}
%            \item first asynchronous federated learning algorithms for vertically partitioned data.
%        \end{itemize}
        
%2021 Peer-to-Peer Networking and Applications: Privacy-preserving two-parties logistic regression on vertically partitioned data using asynchronous gradient sharing~\cite{wei2021privacy}
%        \begin{itemize}
%            \item a protocol using that can complete the logistic regression modeling of vertically partitioned data by asynchronous gradient sharing.
%        \end{itemize}
        
%2021 KDD: AsySQN: Faster Vertical Federated Learning Algorithms with Better Computation Resource Utilization~\cite{zhang2021asysqn}
%        \begin{itemize}
%            \item address the challenges of communication and computation resource utilization
%            \item an asynchronous stochastic quasi-Newton (AsySQN) framework for VFL
%        \end{itemize}
        
%2021 CIKM: Desirable Companion for Vertical Federated Learning: New Zeroth-Order Gradient Based Algorithm~\cite{zhang2021desirable}
%    	\begin{itemize}
%    		\item zero-order optimization methods for VFL
%    		\item theoretical and empirical guarantee on model privacy and accuracy	
%    	\end{itemize}

%2020 Computer Science and Information Systems: A Homomorphic-encryption-based Vertical Federated Learning Scheme for Risk Management~\cite{ou2020homomorphic}
%        \begin{itemize}
%            \item vertical federated learning system for the for Bayesian machine learning with the homomorphic encryption.
%            \item lots of typos.
%        \end{itemize}

==> sections/directions.tex <==
\section{Novel Directions in VFL \highlight{remove and add to previous sections}}
\label{sec:directions}

The development of vertical federated learning will be full of challenge, since vertical federated learning is in its early phase. In this section, we discuss several challenges, which are also promising research directions.

\subsection{Attack and Defense}
Although the attack and defense methods of HFL have been investigated for a while, the attack and defense methods of VFL is still underexpplored. As VFL being widely utilized in both industry and academy rencently, the attack and defense problem becomes more and more important. We discuss the existing two attacks,~\ie{feature and label inference attacks} in VFL and their corresponding defensive methods.

\subsubsection{Label Inference Attack}
Label inference attack conducted by the passive party aims to leak the labels owned by the active party. Fu~\etal proposed three kinds of label inference attack,~\ie, passive label inference attack, active label inference attack and direct label inference attack, for the vertical neural network model~\cite{fu2022label}. Adeversaries could infer the labels of active party from both the received plaintext gradients and obtained plaintext final model weights. The designed attacks are very effective, although they make the assumption that auxiliary labels are provided for the adversary, which could be unavailable in practice. The paper also indicates the existing defense methods~\eg, noisy gradients, for HFL cannot defend these attacks well. 

\subsubsection{Feature Inference Attack}
Feature inference attack is the direct opposite of the label inference attack. It is performed by the active party and tries to infer the features owned the passive party. Luo~\etal designed three feature inference attacks based on model predictions with no prior information of passive party's data distribution~\cite{luo2021feature}. The proposed attacks are effective for logistic regression, decision tree, even complex models,~\eg, random forest. However, they have a very strong assumption that the active party owns the model parameters corresponding to the features in passive party, which is difficult to achieve in reality. Jiang~\etal proposed a more effective attack based on the same setting~\cite{jiang2022comprehensive}. In addition, they also tried to relieve the assumption from the leakage of passive party's model to the prior knowledge of a small set of auxiliary samples.
        
In our opinion, DP, HE and SMC could alleviate this problem. DP is efficient but could result in accuracy loss, while HE and SMC could seal all the gradients and model weigts but suffer from either computation or communication overhead. The mix protocol,~\eg, Sphinx~\cite{tian2022sphinx}, could be a promising direction for designing defensive methods.

\highlight{TODO: more attack works\cite{li2021label,liu2022clustering,liu2022batch,chen2022graph} and defense works~\cite{yang2022differentially,sun2022label,noble2021differentially,wang2020hybrid,sun2021defending}}

\subsubsection{Membership Attack}
\cite{sun2021vertical}

\subsection{Secure Data Market}
Secure data market is platform where companies and institutions could ``buy'' or ``sell'' data without leaking data privacy. In reality, the requirement of data exchange always exists. However, with the improvement of relevant laws and regulations, such operations gradually become impractical. Federated learning provides a feasible solution to build a secure data market. Participants could server as either a data provider or data consumer. Data from different sources is utilized as well as protected according to the discipline of ``available but invisible''. Vertical federated learning plays an important role in secure data market, since enriching profiles for overlapping users is a more common scenario among companies. Security risks may increase when features of one single participant dominate the whole federated model. Efficiency problems are more severe when the number of involved data sources grows. Furthermore, Incentive mechanism is also very important for the market act properly. \highlight{TODO: explain more about the scalability problem}

%\subsection{Feature Heterogeneity}
%
%Similar as the non-IID problem in HFL~\cite{mcmahan2021advances}, feature heterogeneity can be regarded as a unique distribution problem in vertical federated learning~\cite{huang2019large}.

\subsection{Data and Model Heterogeneity}
The heterogeity of VFL contains two parts,~\ie, data and model heterogeneity. Data heterogeneity could be related to the concept of instance proximity~\cite{huang2019large}, which is the similarity between samples calculated by the features. For traditional machine learning, features are heterogeneous, while instance proximities are homogeneous. However, for VFL, features and instance proximities could be both heterogeneous. For example, users can behave differently over various shopping platforms. Features with heterogeneous features and instance proximities cannot benefit or even harm VFL models.~\highlight{decide whether to maintain data heterogeneity.} Besides, most of the existing vertical federated learning models choose to divide the whole original machine learning model into multiple parts and assign them to different parties. However, there exist a more natural requirement that each party wants to choose a specific type of model according to its comprehension about the local features or even derectly use their original local models. FDML provided an ensemble-based solution, which has no restriction about the model type~\cite{hu2019fdml}. However, the leakage of intermediate results leads to privacy risks. In addition, the utilization of original local model involves the knowledge of transfer learning~\cite{pan2009survey}.

%\subsection{Scalability of Parties}
%
%The number of participants in vertical federated learning is usually small comparing with the horizontal scenario~\cite{niu2020billion}.

%\subsection{Public Dataset For Research}
%
%There is still no public dataset of vertical federated learning for research. On the contrary, many datasets of horizontal federated learning have been made public for research purposes~\cite{chai2020fedeval}.

==> sections/layered_approach.tex <==
\section{Layered Approach}
\label{sec:layered}


\begin{figure*}[htbp]
\centering
\includegraphics[width=0.8\linewidth]{figures/design.pdf}
\caption{The designs of vertical federated learning in a layered approach. From bottom to top, the designs could be divided to five layers~\ie, hardware layer, privacy-preserving primitive layer, secure vertical federated algorithm layer, vertical federated system layer and application layer.}
\label{fig:whole_design}
\end{figure*}

In this section, we introduce the design of vertical federated learning as shown in Fig.~\ref{fig:whole_design}. The overall design could be divided to five layers from bottom to top:

%We categorize the existing VFL works according to their main contributions and Tab.~\ref{tab:contribution}.

%We could observe that the amount of vertical federated learning works increases every year, in Fig.~\ref{fig:timeline_VFL}.

%However, there are relatively fewer VFL works, compared with horizontal federated learning, not to mention other machine learning topics.
%Fig.~\ref{fig:application_VFL} shows us the application area of vertical federated learning. 
%As we can see, ... Furthermore, the public dataset of vertical federated learning

\begin{itemize}
	\item {\bf Hardware design} is the bottom-layer design of vertical federated learning. It contains the design of harware-assisted security and hardware-based acceleration.
	\item {\bf Privacy-preserving primitive design} is constructed on the basis of hardware design. It contains the design of cryptographic primitive and non-cryptographic primitive.
	\item {\bf Secure vertical federated algorithm design} is based on the design of privacy-preserving primitive. It could be divided to secure entity alignment algorithm and secure vertical federated learning algorithm.
	\item {\bf Vertical federated system design} builds on the elaborately designed machine learning algorithm. It includes incentive mechanism, architecture, verification, interpretability and inference. 
	\item {\bf Application design} is at the top of vertical federated learning. It covers different areas,~\eg, finance, healthcare, recommender system, CV \& NLP, telecommunication, other applications.
\end{itemize}

In the following sections, we introduce the details of each layer's design by categorizing and analyzing the state-of-the-date methods.

==> sections/open-sourced.tex <==
\section{Open-sourced Vertical Federated Learning Framework}
\label{sec:open-sourced}

In this section, we introduce the existing open-sourced framework that implement vertical federated learning.

\begin{table*}
\centering
\begin{tabular}{ccccc}
\toprule
	Framework & Supporting scenarios & Supporting algorithms & Adopted secure primitives & Design \\
	\midrule
	FATE & &  &  & \\
	\midrule
	PySyft &  &  &  & \\
	\midrule
	FedML &  &  &  & \\
	\midrule
	PaddleFL &  &  &  & \\
	\midrule
	Fedlearner &  &  &  & \\
	\midrule
	FedLearn-algo &  &  &  & \\
	\bottomrule
\end{tabular}
\caption{Comparison of the existing open-sourced vertical federated learning frameworks.}
\label{tab:open-source}
\end{table*}

FATE (Federated AI Technology Enabler)~\footnote{https://github.com/FederatedAI/FATE} is an open-source project initiated by Webank's AI Department to provide a secure computing framework to support the federated AI ecosystem~\cite{liu2021fate}. It is a cross-silo federated learning framework.
    
PySyft~\footnote{https://github.com/OpenMined/PySyft} decouples private data from model training using Federated Learning, Differential Privacy, and Encrypted Computation (like Multi-Party Computation (MPC) and Homomorphic Encryption (HE)) within the main Deep Learning frameworks like PyTorch and TensorFlow.
    

FedML~\footnote{https://fedml.ai/} is a research library and benchmark for federated machine learning.

PaddleFL~\footnote{https://github.com/PaddlePaddle/PaddleFL} is an open source federated learning framework based on PaddlePaddle. Researchers can easily replicate and compare different federated learning algorithms with PaddleFL. Developers can also benefit from PaddleFL in that it is easy to deploy a federated learning system in large scale distributed clusters. In PaddleFL, several federated learning strategies will be provided with application in computer vision, natural language processing, recommendation and so on. Application of traditional machine learning training strategies such as Multi-task learning, Transfer Learning in Federated Learning settings will be provided. Based on PaddlePaddle's large scale distributed training and elastic scheduling of training job on Kubernetes, PaddleFL can be easily deployed based on full-stack open sourced software.
	
Fedlearner~\footnote{https://github.com/bytedance/fedlearner} is collaborative machine learning framework that enables joint modeling of data distributed between institutions.

FedLearn-algo~\footnote{https://github.com/fedlearnAI/fedlearn-algo} is a flexible open-source privacy-preserving machine learning platform~\cite{liu2021fedlearn}. It contains federated doubly stochastic kernel learning for vertically partitioned data~\cite{gu2020federated}, privacy-preserving asynchronous vertical federated learning algorithms for multiparty collaborative learning~\cite{gu2021privacy} and federated random forests.

==> sections/related.tex <==
\section{Related Topics}
\label{sec:related}
In this section, we explain two VFL related topics,~\ie, cross-silo federated learning and model parallelism. They are similar but different essentially, compared with VFL.

%\subsection{Topics in Federated Learning}

\subsection{Cross-Silo Federated Learning}
Cross-silo federated learning refers to the federated learning scenario where participants are companies or institutions~\cite{mcmahan2021advances}. On the contrary, the participants of cross-device federated learning are usually mobile devices. The collaborative training among companies could contain horizontally-partitioned data or vertically-partitioned data. Therefore, cross-silo federated learning can be horizontal federated learning or vertical federated learning. Nowadays, cross-silo federated learning is often confused with VFL because the data of cross-silo federated learning is vertically split in most cases. However, these two concepts are different considering definition.

%\subsubsection{Federated Transfer Learning}
%Federated transfer learning is a federated learning category where participants neither have enough overlapping users nor common feature dimensions~\cite{yang2019federated}. Thus, the federated training in this case is much more difficult. Liu~\textit{et al.} provide a solution to address this problem~\cite{liu2020secure}, which utilizes the small number of overlapping users as a bridge to transfer knowledge from active party with labels to the passive party without labels. On the contrary, the direction of knowledge flow is~\highlight{reverse} with the one of VFL. In vertical federated learning, it is the passive party that provides auxiliary features to help active party train a better model. Therefore, the knowledge is transferred from the former one to the latter one.
    
%\subsubsection{Personalized Federated Learning}

%\subsubsection{Federated Multi-Task Learning}
%Federated multi-task learning~\cite{smith2017federated}. It could be an extension of current VFL because there is only one party holding the label and only one prediction task to complete in the vertical federated scenario. Vertical federated multi-task learning could be regarded as personalized federated learning in the VFL setting. Personalized federated learning is a novel federated learning direction to address data distribution and device capability heterogeneity across data owners~\cite{tan2021towards}.

\subsection{Model Parallelism}
Model parallelism is one of the conventional distributed machine learning methods, which splits data over the feature dimension~\cite{shen2020distributed,liu2021distributed}. Therefore, model parallelism is also known as feature-distributed learning~\cite{zhang2018feature}. As we all know, federated learning can be regarded as the privacy-preserving distributed machine learning. More specifically, VFL corresponds to the privacy-preserving model parallelism~\cite{liu2021distributed}. Compared to data parallelism which splits data over the sample dimension, model parallelism is much less utlized The reasons are: 1) the bottleneck of traditional distributed learning is large amount of data but not large model in most cases; 2) model parallelism is much more complicated than data parallelism because one needs to split the whole model~\cite{vepakomma2018split}. VFL could be a natural scenario where we apply the techniques of model parallelism.
